Tailored Speckle Illumination Microscopy with Enhanced Sectioning and Image Quality

Optical speckle patterns have been widely used for illumination in computational imaging, optical sectioning microscopy, and super-resolution imaging. However, commonly used speckles satisfy Rayleigh statistics, which are not ideal for diverse imaging applications. Here we tailor three-dimensional speckle intensity statistics for dynamic speckle illumination microscopy based on linear fluorescence. Optical sectioning is enhanced by axially varying speckle contrast, and image reconstruction noise is minimized with in-focus speckles of binary intensities. The customized speckle statistics are shown to tolerate sample-induced aberration and scattering. We apply tailored speckle illumination to mouse brain vascular imaging and demonstrate much improved image quality than optical-sectioning structured illumination. These results establish customization of speckle intensity statistics as a promising strategy for robust, high-throughput fluorescence imaging in thick, scattering biological specimens.

==> latexmkrc <==
$out_dir = ".";
$aux_dir = ".";

add_cus_dep('tex', 'aux', 0, 'makeexternaldocument');

sub makeexternaldocument {
    my ($base) = @_;

    # Prevent infinite recursion: main -> supplementary -> main -> ...
    return if $ENV{NO_XR_RECURSE};
    local $ENV{NO_XR_RECURSE} = 1;

    system("latexmk -cd -pdf \"$base\"");
}

